On the Security Vulnerabilities of Text-to-SQL Models

Although it has been demonstrated that Natural Language Processing (NLP) algorithms are vulnerable to deliberate attacks, the question of whether such weaknesses can lead to software security threats is under-explored. To bridge this gap, we conducted vulnerability tests on Text-to-SQL systems that are commonly used to create natural language interfaces to databases. We showed that the Text-to-SQL modules within six commercial applications can be manipulated to produce malicious code, potentially leading to data breaches and Denial of Service attacks. This is the first demonstration that NLP models can be exploited as attack vectors in the wild. In addition, experiments using four open-source language models verified that straightforward backdoor attacks on Text-to-SQL systems achieve a 100% success rate without affecting their performance. The aim of this work is to draw the community's attention to potential software security issues associated with NLP algorithms and encourage exploration of methods to mitigate against them.

==> screenshot/asi2sql/ai2sql_screenshots.tex <==
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/user.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/version.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/database.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/drop.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/benchmark.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/order_repeat.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/houses.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/phoenix.png}
    \end{subfigure}
    ~
    \begin{subfigure}{0.98\textwidth}
    \includegraphics[width=\textwidth]{screenshot/ai2sql/self_injection.png}
    \end{subfigure}
\end{figure}
